Multi-View Neural Surface Reconstruction with Structured Light

Three-dimensional (3D) object reconstruction based on differentiable rendering (DR) is an active research topic in computer vision. DR-based methods minimize the difference between the rendered and target images by optimizing both the shape and appearance and realizing a high visual reproductivity. However, most approaches perform poorly for textureless objects because of the geometrical ambiguity, which means that multiple shapes can have the same rendered result in such objects. To overcome this problem, we introduce active sensing with structured light (SL) into multi-view 3D object reconstruction based on DR to learn the unknown geometry and appearance of arbitrary scenes and camera poses. More specifically, our framework leverages the correspondences between pixels in different views calculated by structured light as an additional constraint in the DR-based optimization of implicit surface, color representations, and camera poses. Because camera poses can be optimized simultaneously, our method realizes high reconstruction accuracy in the textureless region and reduces efforts for camera pose calibration, which is required for conventional SL-based methods. Experiment results on both synthetic and real data demonstrate that our system outperforms conventional DR- and SL-based methods in a high-quality surface reconstruction, particularly for challenging objects with textureless or shiny surfaces.

==> s2_related_work.tex <==
 \vspace{-0.5em}
\section{Related work}

This section briefly reviews the existing approaches to our two key components: 3D reconstruction by structured light and differentiable rendering with neural fields.

% \subsection{Structured light}
\vspace{1mm}
\noindent {\bf Structured light:}
The structured-light technique is widely used to scan the 3D shape of an object, as summarized in detail elsewhere~\cite{Caspi,GuQ,Nguyen,Salvi}.
The scanning process of the structured-light technique involves the projection of a series of known patterns onto the object being scanned while capturing the scene from one or more calibrated cameras. The 3D shape of the object can then be computed by identifying the correspondences between the pixels in the images captured by the camera(s). To find these correspondences, the projected pattern is encoded such that every pixel in the projected pattern can be uniquely identified in the images captured by the cameras. This provides an efficient and highly accurate method to map the corresponding pixels between images captured by cameras. 
These methods can achieve high-quality reconstruction irrespective of surface textures~\cite{Aliaga,Geng,inokuchi1984range,Michael}.
To obtain the entire shape of an object, there are two common approaches to align the multiple scans from different viewpoints (camera and projector pairs) into a single global coordinate.
One approach~\cite{sadlo2005practical,sainz2004simple} is to obtain the global camera poses using markers fixed with the object.
The other approach~\cite{furuakwa2009multi,furukawa2019simultaneous} is to register all point cloud parts using the iterative closest point~(ICP) method~\cite{icp}.
However, both approaches lead to registration error.
% To obtain the entire shape of an object, a common approach~\cite{furuakwa2009multi,furukawa2019simultaneous} is to align the multiple scans from different viewpoints (camera and projector pairs) into a single global coordinate using the iterative closest point~(ICP) method~\cite{icp}. However, ICP alignment is unreliable when an object has repetitive structures or no distinctive 3D structures.
Recently, some multi-view structured light methods~\cite{Furukawa2,Garrido,li2019pro,Li7} have realized self-calibrating reconstruction of 3D points. The key to these methods is that the structured light patterns projected by one fixed projector are captured from more than two camera viewpoints with viewing angle overlaps, so that feature matching and tracking can be performed to connect all projectors and cameras.
However, objects with shiny surfaces are difficult to be measured accurately using these conventional structured-light methods because the shiny surfaces result in the appearance of highlights and inter-reflections in the captured images, which causes measurement errors.

% \subsection{Differentiable rendering-based surface reconstruction}
\vspace{1mm}
\noindent {\bf Differentiable rendering-based 3D reconstruction:}
Using differentiable rendering (DR)~\cite{kato2020differentiable,zhao2020physics}, scene geometries can be estimated by minimizing the difference between rendered and input images. One promising 3D representation is neural fields~\cite{neuralfields}, which model geometry and appearance by multi-layer perceptrons (MLPs), because they can represent 3D content continuously without discretization.
After the optimization, a triangular mesh can be directly extracted from the neural implicit functions.
The neural implicit functions can be roughly classified into two categories, including density/transparency fields, which are adopted by NeRF~\cite{nerf} and in follow-up works~\cite{boss2021nerd,martin2021nerf,neff2021donerf,niemeyer2021giraffe,peng2021neural,pumarola2021d}, and implicit surfaces, such as occupancy functions~\cite{mescheder2019occupancy,dvr} and signed distance functions (SDFs)~\cite{liu2020dist,liu2019learning,idr}.
Although density/transparency fields have shown impressive results in novel view synthesis, their surfaces extracted as level sets of the underlying volume density are usually non-smooth and contain artifacts owing to the flexibility of the radiance field representation~\cite{unisurf}.
By contrast, the occupancy function and SDF provide smoother and cleaner surface results by explicitly defining the surfaces of objects and optimizing the surfaces directly.
UNISURF~\cite{unisurf}, NeuS~\cite{neus}, and VolSDF~\cite{volsdf} improved the rendering approach for the occupancy function and SDF and achieved higher-quality 3D reconstruction.
However, the geometry ambiguity problem in observations, as described in Section~\ref{sec:introduction}, remains unsolved; therefore, these methods are unstable when reconstructing  surfaces with few textures.
More recently, Zhang et al.~\cite{zhang2021learning} leveraged the knowledge of stereo matching and feature consistency to optimize an implicit surface representation. However, this method is based on local feature extraction, which is also unreliable for textureless scenes.
In this study, we propose a robust approach to solving the geometrical ambiguity problem by introducing dense and accurate correspondences extracted from structured light as supervision, which are independent of the original textures of objects.
